Quantum fluctuation of ferroelectric order in polar metals

Since its discovery a decade ago, "polar metallic phase" has ignited significant research interest, as it further functionalizes the switchable electric polarization of materials with additional transport capability, granting them great potential in next-generation electronic devices. The polar metallic phase is an unusual metallic phase of matter containing long-range ferroelectric (FE) order in the electronic and atomic structure. Distinct from the typical FE insulating phase, this phase spontaneously breaks the inversion symmetry but without global polarization. Unexpectedly, the FE order is found to be dramatically suppressed by carriers and destroyed at moderate ~10% carrier density. Here, we propose a general mechanism based on carrier-induced quantum fluctuations to explain this puzzling phenomenon. Basically, the quantum kinetic effect would drive the formation of polaronic quasi-particles made of the carriers and their surrounding dipoles. The disruption in dipolar directions can therefore weaken or even destroy the FE order. We demonstrate such polaron formation and the associated FE suppression via a simple model using exact diagonalization, perturbation, and quantum Monte Carlo approaches. This quantum mechanism also provides an intuitive picture for many puzzling experimental findings, thereby facilitating new designs of multifunctional FE electronic devices augmented with quantum effects.

==> Quantum fluctuation of ferroelectric order in polar metals/eg1.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(130.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,82){\makebox(0,0)[r]{$-1$}}
\put(1419.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,276){\makebox(0,0)[r]{$-0.5$}}
\put(1419.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,470.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,470){\makebox(0,0)[r]{$0$}}
\put(1419.0,470.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,664.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,664){\makebox(0,0)[r]{$0.5$}}
\put(1419.0,664.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,858.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,858){\makebox(0,0)[r]{$1$}}
\put(1419.0,858.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(159.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(159,41){\makebox(0,0){$-3$}}
\put(159.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(368.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(368,41){\makebox(0,0){$-2$}}
\put(368.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(576.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(576,41){\makebox(0,0){$-1$}}
\put(576.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(785.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(785,41){\makebox(0,0){$0$}}
\put(785.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(993.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(993,41){\makebox(0,0){$1$}}
\put(993.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1201.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1201,41){\makebox(0,0){$2$}}
\put(1201.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1410.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1410,41){\makebox(0,0){$3$}}
\put(1410.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(130.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,82.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,858.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(368,664){\makebox(0,0){$erf(x) = \frac{2}{\sqrt{\pi}}\int_0^x\, dt e^{-t^2}$}}
\put(1279,817){\makebox(0,0)[r]{sin(x)}}
\put(1299.0,817.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(130,469){\usebox{\plotpoint}}
\multiput(130.58,465.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(129.17,467.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(143.58,441.39)(0.493,-0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(142.17,443.20)(13.000,-23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(156.58,416.74)(0.494,-0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(155.17,418.37)(14.000,-22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(170.58,392.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(169.17,394.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(183.58,368.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(182.17,370.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(196.58,344.65)(0.493,-0.893){23}{\rule{0.119pt}{0.808pt}}
\multiput(195.17,346.32)(13.000,-21.324){2}{\rule{0.400pt}{0.404pt}}
\multiput(209.58,321.98)(0.494,-0.791){25}{\rule{0.119pt}{0.729pt}}
\multiput(208.17,323.49)(14.000,-20.488){2}{\rule{0.400pt}{0.364pt}}
\multiput(223.58,299.77)(0.493,-0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(222.17,301.39)(13.000,-20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(236.58,277.90)(0.493,-0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(235.17,279.45)(13.000,-19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(249.58,257.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(248.17,258.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(262.58,237.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(261.17,238.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(275.58,217.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(274.17,218.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(289.58,199.41)(0.493,-0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(288.17,200.71)(13.000,-15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(302.58,182.54)(0.493,-0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(301.17,183.77)(13.000,-14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(315.58,166.67)(0.493,-0.576){23}{\rule{0.119pt}{0.562pt}}
\multiput(314.17,167.83)(13.000,-13.834){2}{\rule{0.400pt}{0.281pt}}
\multiput(328.00,152.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(328.00,153.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(342.00,138.92)(0.539,-0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(342.00,139.17)(11.893,-12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(355.00,126.92)(0.590,-0.492){19}{\rule{0.573pt}{0.118pt}}
\multiput(355.00,127.17)(11.811,-11.000){2}{\rule{0.286pt}{0.400pt}}
\multiput(368.00,115.92)(0.652,-0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(368.00,116.17)(11.713,-10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(381.00,105.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(381.00,106.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(394.00,97.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(394.00,98.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(408.00,91.93)(1.378,-0.477){7}{\rule{1.140pt}{0.115pt}}
\multiput(408.00,92.17)(10.634,-5.000){2}{\rule{0.570pt}{0.400pt}}
\multiput(421.00,86.94)(1.797,-0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(421.00,87.17)(10.094,-4.000){2}{\rule{0.700pt}{0.400pt}}
\put(434,82.17){\rule{2.700pt}{0.400pt}}
\multiput(434.00,83.17)(7.396,-2.000){2}{\rule{1.350pt}{0.400pt}}
\put(461,81.67){\rule{3.132pt}{0.400pt}}
\multiput(461.00,81.17)(6.500,1.000){2}{\rule{1.566pt}{0.400pt}}
\multiput(474.00,83.61)(2.695,0.447){3}{\rule{1.833pt}{0.108pt}}
\multiput(474.00,82.17)(9.195,3.000){2}{\rule{0.917pt}{0.400pt}}
\multiput(487.00,86.60)(1.797,0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(487.00,85.17)(10.094,4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(500.00,90.59)(1.123,0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(500.00,89.17)(10.994,6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(513.00,96.59)(1.026,0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(513.00,95.17)(12.132,7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(527.00,103.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(527.00,102.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(540.00,112.58)(0.652,0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(540.00,111.17)(11.713,10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(553.00,122.58)(0.539,0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(553.00,121.17)(11.893,12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(566.00,134.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(566.00,133.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(580.58,147.00)(0.493,0.536){23}{\rule{0.119pt}{0.531pt}}
\multiput(579.17,147.00)(13.000,12.898){2}{\rule{0.400pt}{0.265pt}}
\multiput(593.58,161.00)(0.493,0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(592.17,161.00)(13.000,14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(606.58,177.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(605.17,177.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(619.58,194.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(618.17,194.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(632.58,211.00)(0.494,0.680){25}{\rule{0.119pt}{0.643pt}}
\multiput(631.17,211.00)(14.000,17.666){2}{\rule{0.400pt}{0.321pt}}
\multiput(646.58,230.00)(0.493,0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(645.17,230.00)(13.000,18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(659.58,250.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(658.17,250.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(672.58,271.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(671.17,271.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(685.58,292.00)(0.494,0.827){25}{\rule{0.119pt}{0.757pt}}
\multiput(684.17,292.00)(14.000,21.429){2}{\rule{0.400pt}{0.379pt}}
\multiput(699.58,315.00)(0.493,0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(698.17,315.00)(13.000,20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(712.58,337.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(711.17,337.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(725.58,361.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(724.17,361.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(738.58,385.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(737.17,385.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(751.58,409.00)(0.494,0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(750.17,409.00)(14.000,22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(765.58,433.00)(0.493,0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(764.17,433.00)(13.000,23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(778.58,458.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(777.17,458.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(791.58,482.00)(0.493,0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(790.17,482.00)(13.000,23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(804.58,507.00)(0.494,0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(803.17,507.00)(14.000,22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(818.58,531.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(817.17,531.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(831.58,555.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(830.17,555.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(844.58,579.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(843.17,579.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(857.58,603.00)(0.493,0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(856.17,603.00)(13.000,20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(870.58,625.00)(0.494,0.827){25}{\rule{0.119pt}{0.757pt}}
\multiput(869.17,625.00)(14.000,21.429){2}{\rule{0.400pt}{0.379pt}}
\multiput(884.58,648.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(883.17,648.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(897.58,669.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(896.17,669.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(910.58,690.00)(0.493,0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(909.17,690.00)(13.000,18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(923.58,710.00)(0.494,0.680){25}{\rule{0.119pt}{0.643pt}}
\multiput(922.17,710.00)(14.000,17.666){2}{\rule{0.400pt}{0.321pt}}
\multiput(937.58,729.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(936.17,729.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(950.58,746.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(949.17,746.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(963.58,763.00)(0.493,0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(962.17,763.00)(13.000,14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(976.58,779.00)(0.493,0.536){23}{\rule{0.119pt}{0.531pt}}
\multiput(975.17,779.00)(13.000,12.898){2}{\rule{0.400pt}{0.265pt}}
\multiput(989.00,793.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(989.00,792.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(1003.00,806.58)(0.539,0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(1003.00,805.17)(11.893,12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(1016.00,818.58)(0.652,0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(1016.00,817.17)(11.713,10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(1029.00,828.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(1029.00,827.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(1042.00,837.59)(1.026,0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(1042.00,836.17)(12.132,7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(1056.00,844.59)(1.123,0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(1056.00,843.17)(10.994,6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(1069.00,850.60)(1.797,0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(1069.00,849.17)(10.094,4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(1082.00,854.61)(2.695,0.447){3}{\rule{1.833pt}{0.108pt}}
\multiput(1082.00,853.17)(9.195,3.000){2}{\rule{0.917pt}{0.400pt}}
\put(1095,856.67){\rule{3.132pt}{0.400pt}}
\multiput(1095.00,856.17)(6.500,1.000){2}{\rule{1.566pt}{0.400pt}}
\put(447.0,82.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\put(1122,856.17){\rule{2.700pt}{0.400pt}}
\multiput(1122.00,857.17)(7.396,-2.000){2}{\rule{1.350pt}{0.400pt}}
\multiput(1135.00,854.94)(1.797,-0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(1135.00,855.17)(10.094,-4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(1148.00,850.93)(1.378,-0.477){7}{\rule{1.140pt}{0.115pt}}
\multiput(1148.00,851.17)(10.634,-5.000){2}{\rule{0.570pt}{0.400pt}}
\multiput(1161.00,845.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(1161.00,846.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(1175.00,839.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(1175.00,840.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(1188.00,831.92)(0.652,-0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(1188.00,832.17)(11.713,-10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(1201.00,821.92)(0.590,-0.492){19}{\rule{0.573pt}{0.118pt}}
\multiput(1201.00,822.17)(11.811,-11.000){2}{\rule{0.286pt}{0.400pt}}
\multiput(1214.00,810.92)(0.539,-0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(1214.00,811.17)(11.893,-12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(1227.00,798.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(1227.00,799.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(1241.58,783.67)(0.493,-0.576){23}{\rule{0.119pt}{0.562pt}}
\multiput(1240.17,784.83)(13.000,-13.834){2}{\rule{0.400pt}{0.281pt}}
\multiput(1254.58,768.54)(0.493,-0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(1253.17,769.77)(13.000,-14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(1267.58,752.41)(0.493,-0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(1266.17,753.71)(13.000,-15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(1280.58,735.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(1279.17,736.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(1294.58,717.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(1293.17,718.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(1307.58,697.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(1306.17,698.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(1320.58,676.90)(0.493,-0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(1319.17,678.45)(13.000,-19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(1333.58,655.77)(0.493,-0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(1332.17,657.39)(13.000,-20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(1346.58,633.98)(0.494,-0.791){25}{\rule{0.119pt}{0.729pt}}
\multiput(1345.17,635.49)(14.000,-20.488){2}{\rule{0.400pt}{0.364pt}}
\multiput(1360.58,611.65)(0.493,-0.893){23}{\rule{0.119pt}{0.808pt}}
\multiput(1359.17,613.32)(13.000,-21.324){2}{\rule{0.400pt}{0.404pt}}
\multiput(1373.58,588.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1372.17,590.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1386.58,564.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1385.17,566.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1399.58,540.74)(0.494,-0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(1398.17,542.37)(14.000,-22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(1413.58,516.39)(0.493,-0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(1412.17,518.20)(13.000,-23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(1426.58,491.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1425.17,493.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\put(1108.0,858.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\put(130.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,82.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,858.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\end{picture}


==> Quantum fluctuation of ferroelectric order in polar metals/jie_QMCpart.tex <==
\item \textit{World-line quantum Monte Carlo (QMC)}: We use QMC to measure the thermal average of the FE order $\langle \mathrm{\mathbf{O}}\rangle$ at finite temperatures. 
The $H_{R}$ term in Hamiltonian (Eq.\ref{eqn:total_hamil}) is not included in order to study the quantum effect only. 
The FE order can be written as $\langle \mathrm{\mathbf{O}}\rangle=\frac 1 Z \Tr (\mathrm{\mathbf{O}}\ \mathrm{exp} (-\beta H) )$, where $H$ is the Hamiltonian, $\beta=1/(k_B T)$ is the inverse temperature, and $Z=\Tr (\mathrm{exp}(-\beta H))$ is the partition function.


In our QMC calculation, the basis is taken as $c_i^\dagger\prod_{j}a^\dagger_{j n_j}|0\rangle$. The dimension of Hilbert space is $8^{L^3-1}\times L$ where $L$ is the system size. 
The Hamiltonian can be written in terms of $H=T+H_0$, where $H_0$ is the diagonal part and $T$ is the non-diagonal part. 
Using an interaction picture, we can represent the Boltzmann factor as $\exp{(-\beta H)}=\exp{(-\beta H_0)}\sum_{k=0}^\infty (-1)^k \int_0^\beta \,\mathrm{d}\tau_1\int_0^{\tau_1}\,\mathrm{d}\tau_2\cdots\int_0^{\tau_{k-1}}\,\mathrm{d}\tau_k V_{\tau_1}^D V_{\tau_2}^D\cdots V_{\tau_k}^D$ where $V_{\tau_i}^D=\exp{(\tau_i H_0)}V\exp{(-\tau_i H_0)}$. 
Here we treat $\tau$ as the imaginary time and plug complete relations between each $V_{\tau_i}^D$, then $\langle \mathrm{\mathbf{O}}\rangle$ can be treated as a weighted average among all possible closed paths (world line) in space-time. The non-diagonal term (the kinetic part) leads to a ``hop'' between lattice sites, thus creating a ``kink'' on the world line. 
Importance sampling is done through the Metropolis algorithm. Ergodicity and detailed balance ensure the sequence of world lines converges to the desired distribution. 
%In principle, a global update scheme must be applied to generate different topological structures of paths. 
%However, in our study, the additional freedom in the dipole orientation makes it hard to generate a non-trivial topological structure in the phase space, because the electron must recover the dipole configuration after it comes back. Therefore, local update schemes are already a very good approximation, which consists of two schemes-- creation/annihilation of ``kink-antikink" pair and the time shift of kinks. 


We use an in-house MATLAB code for the world-line QMC calculations, with a $5\times5\times5$ supercell under periodic boundary conditions. 
The supercell size used was tested by a system size scaling as shown in Fig.~\ref{fig:supple_QMC}(a).
%Same to the above two approaches, all local dipoles are aligned with a single carrier introduced as the lowest energy starting configuration. 
At every kink point, we store the imaginary time, the electron position, and the dipole configuration as matrices, and build a mapping between them. The weight of the paths and the estimator can be calculated from these matrices. 
In the update scheme, we generate a random kink-antikink pair at $\tau_1$ and $\tau_2$. Between these two time points, we propose a carrier hopping to one of the neighboring sites, randomly leaving a dipole orientation at the original site. Then, we shift the kink from $\tau_1$ to $\tau_2$ correspondingly. 
We accept these updates with certain probabilities obtained from the detailed balance. 
Through this scheme, the system gradually converges to its thermally equilibrated state.
The calculation only converges fast at high temperatures $(k_B T)/J>0.1$, below which the acceptance ratio becomes exponentially small. 
%In the region of $(k_B T)<J$, the broken inversion symmetry is well preserved in a long timescale, because it consumes considerable energy to globally flip the local dipoles. 

%Different from the ground state study of the formation of the polaron, the finite temperature calculations provide us with a thermodynamically equilibrated Bloch-state, which involves the effect of the low-energy kinetic process of the polaron as a quasi-particle. 
%The further effect of the polaron ``tail" to the FE order and the lack of the thermal effects to self-correct the local dipoles lead to a larger $N_{\mathbf{p}}$ in QMC simulations compared to those obtained from ED and perturbation approaches.
As shown in Fig.~\ref{fig:supple_QMC}(b), $N_{\mathbf{p}}$ slightly decreases as $T$ increases in the low-$T$ range.
%This slight Np decrease is because with the increase of $T$, the thermal distribution suppresses the effect of the virtual kinetic process by averaging thermodynamically equilibrated Bloch states into a localized-like state, therefore $N_{\mathbf{p}}$ slightly decreases with temperature.
The slight decrease in $N_{\mathbf{p}}$ is attributed to the rise in temperature, which causes the thermal distribution to suppress the impact of the virtual kinetic process by averaging out thermodynamically equilibrated Bloch states into a localized state.
Fig.~\ref{fig:supple_QMC}(b) also showcases the dominance of thermal fluctuations over quantum fluctuations in the high-temperature range.
%demonstrates the dominance of the thermal fluctuation over the quantum fluctuation in the relative high-$T$ range.
%Already defined Np
%The projection of dipoles along [111] direction is statistically averaged in our simulation, as a measurement of polaron size at finite temperature.

\begin{figure}[!h]
\includegraphics[width=0.8\columnwidth]{supple2.png}
\centering
\caption{
(a) The $t/J$ dependence of $N_{\mathbf{p}}$ at various cubic system size $L^3$ for $L=5,6,7,8$ under a fixed finite temperature $k_{B}T/J=0.2$; (b) Temperature dependence of $N_{\mathbf{p}}$ for different $t/J$ parameter.
}
\label{fig:supple_QMC}
\end{figure}



%The above dynamical effects of the polaron and the finite-temperature effects are studied through a world-line QMC approach.
%Note that the self-correction term ($H_R$) is not included in the Hamiltonian, which means the local dipoles can not be reoriented by merely thermal effects.
%(This exclusion of $H_R$ term clearly separates the quantum effects with the thermal ones, thereby enables us to focus on the quantum virtual kinetic process only.
%If we put back the thermal fluctuations of local dipoles, we could clearly see the thermal effects being supplemented, gradually dominating over the quantum effects with increasing temperature.)


%This renormalized kinetic effect is more predominant at higher $t/J$, which vanishes as $t/J\rightarrow 0$.
%This is clearly shown in Fig.~\ref{fig:dipole_result}(c).
%This effect further strengthens our argument that the polaron formation could effectively suppress the FE order, and even lower the critical $x_c$.)
%According to Fig.~\ref{fig:dipole_result}(c), same as the other methods, the quantum fluctuation effect in QMC calculation is more prominent with larger polaron formed at larger $t/J$ value, regardless of the temperature.
%Moreover, as shown in Fig.~\ref{fig:dipole_result}(e), $N_{\mathbf{p}}$ slightly decreases as $T$ increases in the low-$T$ range.
%With the increase of $T$, the thermal distribution suppresses the effect of the virtual kinetic process by averaging all those Bloch states into a localized-like state, therefore $N_{\mathbf{p}}$ slightly decreases with temperature.
%Fig.~\ref{fig:dipole_result}(e) also demonstrates the dominance of the thermal fluctuation over the quantum fluctuation at the high-$T$ range.

==> eg1.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(130.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,82){\makebox(0,0)[r]{$-1$}}
\put(1419.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,276){\makebox(0,0)[r]{$-0.5$}}
\put(1419.0,276.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,470.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,470){\makebox(0,0)[r]{$0$}}
\put(1419.0,470.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,664.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,664){\makebox(0,0)[r]{$0.5$}}
\put(1419.0,664.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(130.0,858.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(110,858){\makebox(0,0)[r]{$1$}}
\put(1419.0,858.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(159.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(159,41){\makebox(0,0){$-3$}}
\put(159.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(368.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(368,41){\makebox(0,0){$-2$}}
\put(368.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(576.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(576,41){\makebox(0,0){$-1$}}
\put(576.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(785.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(785,41){\makebox(0,0){$0$}}
\put(785.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(993.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(993,41){\makebox(0,0){$1$}}
\put(993.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1201.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1201,41){\makebox(0,0){$2$}}
\put(1201.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1410.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1410,41){\makebox(0,0){$3$}}
\put(1410.0,838.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(130.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,82.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,858.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(368,664){\makebox(0,0){$erf(x) = \frac{2}{\sqrt{\pi}}\int_0^x\, dt e^{-t^2}$}}
\put(1279,817){\makebox(0,0)[r]{sin(x)}}
\put(1299.0,817.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(130,469){\usebox{\plotpoint}}
\multiput(130.58,465.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(129.17,467.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(143.58,441.39)(0.493,-0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(142.17,443.20)(13.000,-23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(156.58,416.74)(0.494,-0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(155.17,418.37)(14.000,-22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(170.58,392.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(169.17,394.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(183.58,368.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(182.17,370.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(196.58,344.65)(0.493,-0.893){23}{\rule{0.119pt}{0.808pt}}
\multiput(195.17,346.32)(13.000,-21.324){2}{\rule{0.400pt}{0.404pt}}
\multiput(209.58,321.98)(0.494,-0.791){25}{\rule{0.119pt}{0.729pt}}
\multiput(208.17,323.49)(14.000,-20.488){2}{\rule{0.400pt}{0.364pt}}
\multiput(223.58,299.77)(0.493,-0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(222.17,301.39)(13.000,-20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(236.58,277.90)(0.493,-0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(235.17,279.45)(13.000,-19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(249.58,257.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(248.17,258.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(262.58,237.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(261.17,238.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(275.58,217.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(274.17,218.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(289.58,199.41)(0.493,-0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(288.17,200.71)(13.000,-15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(302.58,182.54)(0.493,-0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(301.17,183.77)(13.000,-14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(315.58,166.67)(0.493,-0.576){23}{\rule{0.119pt}{0.562pt}}
\multiput(314.17,167.83)(13.000,-13.834){2}{\rule{0.400pt}{0.281pt}}
\multiput(328.00,152.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(328.00,153.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(342.00,138.92)(0.539,-0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(342.00,139.17)(11.893,-12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(355.00,126.92)(0.590,-0.492){19}{\rule{0.573pt}{0.118pt}}
\multiput(355.00,127.17)(11.811,-11.000){2}{\rule{0.286pt}{0.400pt}}
\multiput(368.00,115.92)(0.652,-0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(368.00,116.17)(11.713,-10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(381.00,105.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(381.00,106.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(394.00,97.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(394.00,98.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(408.00,91.93)(1.378,-0.477){7}{\rule{1.140pt}{0.115pt}}
\multiput(408.00,92.17)(10.634,-5.000){2}{\rule{0.570pt}{0.400pt}}
\multiput(421.00,86.94)(1.797,-0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(421.00,87.17)(10.094,-4.000){2}{\rule{0.700pt}{0.400pt}}
\put(434,82.17){\rule{2.700pt}{0.400pt}}
\multiput(434.00,83.17)(7.396,-2.000){2}{\rule{1.350pt}{0.400pt}}
\put(461,81.67){\rule{3.132pt}{0.400pt}}
\multiput(461.00,81.17)(6.500,1.000){2}{\rule{1.566pt}{0.400pt}}
\multiput(474.00,83.61)(2.695,0.447){3}{\rule{1.833pt}{0.108pt}}
\multiput(474.00,82.17)(9.195,3.000){2}{\rule{0.917pt}{0.400pt}}
\multiput(487.00,86.60)(1.797,0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(487.00,85.17)(10.094,4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(500.00,90.59)(1.123,0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(500.00,89.17)(10.994,6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(513.00,96.59)(1.026,0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(513.00,95.17)(12.132,7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(527.00,103.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(527.00,102.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(540.00,112.58)(0.652,0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(540.00,111.17)(11.713,10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(553.00,122.58)(0.539,0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(553.00,121.17)(11.893,12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(566.00,134.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(566.00,133.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(580.58,147.00)(0.493,0.536){23}{\rule{0.119pt}{0.531pt}}
\multiput(579.17,147.00)(13.000,12.898){2}{\rule{0.400pt}{0.265pt}}
\multiput(593.58,161.00)(0.493,0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(592.17,161.00)(13.000,14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(606.58,177.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(605.17,177.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(619.58,194.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(618.17,194.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(632.58,211.00)(0.494,0.680){25}{\rule{0.119pt}{0.643pt}}
\multiput(631.17,211.00)(14.000,17.666){2}{\rule{0.400pt}{0.321pt}}
\multiput(646.58,230.00)(0.493,0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(645.17,230.00)(13.000,18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(659.58,250.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(658.17,250.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(672.58,271.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(671.17,271.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(685.58,292.00)(0.494,0.827){25}{\rule{0.119pt}{0.757pt}}
\multiput(684.17,292.00)(14.000,21.429){2}{\rule{0.400pt}{0.379pt}}
\multiput(699.58,315.00)(0.493,0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(698.17,315.00)(13.000,20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(712.58,337.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(711.17,337.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(725.58,361.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(724.17,361.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(738.58,385.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(737.17,385.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(751.58,409.00)(0.494,0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(750.17,409.00)(14.000,22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(765.58,433.00)(0.493,0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(764.17,433.00)(13.000,23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(778.58,458.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(777.17,458.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(791.58,482.00)(0.493,0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(790.17,482.00)(13.000,23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(804.58,507.00)(0.494,0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(803.17,507.00)(14.000,22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(818.58,531.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(817.17,531.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(831.58,555.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(830.17,555.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(844.58,579.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(843.17,579.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(857.58,603.00)(0.493,0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(856.17,603.00)(13.000,20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(870.58,625.00)(0.494,0.827){25}{\rule{0.119pt}{0.757pt}}
\multiput(869.17,625.00)(14.000,21.429){2}{\rule{0.400pt}{0.379pt}}
\multiput(884.58,648.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(883.17,648.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(897.58,669.00)(0.493,0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(896.17,669.00)(13.000,19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(910.58,690.00)(0.493,0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(909.17,690.00)(13.000,18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(923.58,710.00)(0.494,0.680){25}{\rule{0.119pt}{0.643pt}}
\multiput(922.17,710.00)(14.000,17.666){2}{\rule{0.400pt}{0.321pt}}
\multiput(937.58,729.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(936.17,729.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(950.58,746.00)(0.493,0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(949.17,746.00)(13.000,15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(963.58,763.00)(0.493,0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(962.17,763.00)(13.000,14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(976.58,779.00)(0.493,0.536){23}{\rule{0.119pt}{0.531pt}}
\multiput(975.17,779.00)(13.000,12.898){2}{\rule{0.400pt}{0.265pt}}
\multiput(989.00,793.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(989.00,792.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(1003.00,806.58)(0.539,0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(1003.00,805.17)(11.893,12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(1016.00,818.58)(0.652,0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(1016.00,817.17)(11.713,10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(1029.00,828.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(1029.00,827.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(1042.00,837.59)(1.026,0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(1042.00,836.17)(12.132,7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(1056.00,844.59)(1.123,0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(1056.00,843.17)(10.994,6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(1069.00,850.60)(1.797,0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(1069.00,849.17)(10.094,4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(1082.00,854.61)(2.695,0.447){3}{\rule{1.833pt}{0.108pt}}
\multiput(1082.00,853.17)(9.195,3.000){2}{\rule{0.917pt}{0.400pt}}
\put(1095,856.67){\rule{3.132pt}{0.400pt}}
\multiput(1095.00,856.17)(6.500,1.000){2}{\rule{1.566pt}{0.400pt}}
\put(447.0,82.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\put(1122,856.17){\rule{2.700pt}{0.400pt}}
\multiput(1122.00,857.17)(7.396,-2.000){2}{\rule{1.350pt}{0.400pt}}
\multiput(1135.00,854.94)(1.797,-0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(1135.00,855.17)(10.094,-4.000){2}{\rule{0.700pt}{0.400pt}}
\multiput(1148.00,850.93)(1.378,-0.477){7}{\rule{1.140pt}{0.115pt}}
\multiput(1148.00,851.17)(10.634,-5.000){2}{\rule{0.570pt}{0.400pt}}
\multiput(1161.00,845.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(1161.00,846.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(1175.00,839.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(1175.00,840.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(1188.00,831.92)(0.652,-0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(1188.00,832.17)(11.713,-10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(1201.00,821.92)(0.590,-0.492){19}{\rule{0.573pt}{0.118pt}}
\multiput(1201.00,822.17)(11.811,-11.000){2}{\rule{0.286pt}{0.400pt}}
\multiput(1214.00,810.92)(0.539,-0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(1214.00,811.17)(11.893,-12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(1227.00,798.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(1227.00,799.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(1241.58,783.67)(0.493,-0.576){23}{\rule{0.119pt}{0.562pt}}
\multiput(1240.17,784.83)(13.000,-13.834){2}{\rule{0.400pt}{0.281pt}}
\multiput(1254.58,768.54)(0.493,-0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(1253.17,769.77)(13.000,-14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(1267.58,752.41)(0.493,-0.655){23}{\rule{0.119pt}{0.623pt}}
\multiput(1266.17,753.71)(13.000,-15.707){2}{\rule{0.400pt}{0.312pt}}
\multiput(1280.58,735.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(1279.17,736.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(1294.58,717.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(1293.17,718.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(1307.58,697.03)(0.493,-0.774){23}{\rule{0.119pt}{0.715pt}}
\multiput(1306.17,698.52)(13.000,-18.515){2}{\rule{0.400pt}{0.358pt}}
\multiput(1320.58,676.90)(0.493,-0.814){23}{\rule{0.119pt}{0.746pt}}
\multiput(1319.17,678.45)(13.000,-19.451){2}{\rule{0.400pt}{0.373pt}}
\multiput(1333.58,655.77)(0.493,-0.853){23}{\rule{0.119pt}{0.777pt}}
\multiput(1332.17,657.39)(13.000,-20.387){2}{\rule{0.400pt}{0.388pt}}
\multiput(1346.58,633.98)(0.494,-0.791){25}{\rule{0.119pt}{0.729pt}}
\multiput(1345.17,635.49)(14.000,-20.488){2}{\rule{0.400pt}{0.364pt}}
\multiput(1360.58,611.65)(0.493,-0.893){23}{\rule{0.119pt}{0.808pt}}
\multiput(1359.17,613.32)(13.000,-21.324){2}{\rule{0.400pt}{0.404pt}}
\multiput(1373.58,588.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1372.17,590.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1386.58,564.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1385.17,566.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1399.58,540.74)(0.494,-0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(1398.17,542.37)(14.000,-22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(1413.58,516.39)(0.493,-0.972){23}{\rule{0.119pt}{0.869pt}}
\multiput(1412.17,518.20)(13.000,-23.196){2}{\rule{0.400pt}{0.435pt}}
\multiput(1426.58,491.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1425.17,493.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\put(1108.0,858.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\put(130.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,82.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\put(1439.0,82.0){\rule[-0.200pt]{0.400pt}{186.938pt}}
\put(130.0,858.0){\rule[-0.200pt]{315.338pt}{0.400pt}}
\end{picture}

